How to Compute Modulo Prime-Power Sums ?

A new class of structured codes called Quasi Group Codes (QGC) is introduced. A QGC is a subset of a group code. In contrast with group codes, QGCs are not closed under group addition. The parameters of the QGC can be chosen such that the size of $\mathcal{C}+\mathcal{C}$ is equal to any number between $|\mathcal{C}|$ and $|\mathcal{C}|^2$ . We analyze the performance of a specific class of QGCs. This class of QGCs is constructed by assigning single-letter distributions to the indices of the codewords in a group code. Then, the QGC is defined as the set of codewords whose index is in the typical set corresponding to these single-letter distributions. The asymptotic performance limits of this class of QGCs is characterized using single-letter information quantities. Corresponding covering and packing bounds are derived. It is shown that the point-to-point channel capacity and optimal rate-distortion function are achievable using QGCs. Coding strategies based on QGCs are introduced for three fundamental multi-terminal problems: the K\"orner-Marton problem for modulo prime-power sums, computation over the multiple access channel (MAC), and MAC with distributed states. For each problem a single-letter achievable rate-region is derived. It is shown, through examples, that the coding strategies improve upon the previous strategies based on unstructured codes, linear codes and group codes.

==> Proof_of_thm_QGC_with_unstructured_codes.tex <==
\section{Proof of Theorem \ref{thm: QGC+unstructured ahcievable}} \label{sec: proof of thm QGC+unstructured achievable}
\begin{proof}
We propose a coding scheme which is a combination of two coding schemes: 1) Gel'fand-Pinsker scheme, and 2) the proposed scheme in Theorem \ref{thm: QGC MAC with state achievable} which is uses nested QGCs. Suppose $M_j$ is the message for the $j$th user. $M_j$ is drawn randomly and uniformly from $[1:2^{R_j}]$. The $j$th encoder splits its message $M_j$ into two parts $M_{j,1}$ and $M_{j,2}$, where $j=1,2$. Suppose $M_{j,1}\in [1: 2^{nR_{j,1}}] $ and $M_{j,2}\in [1: 2^{nR_{j,2}}]$, where $R_j=R_{j,1}+R_{j,2}$. The first part $M_{j,1}$ is encoded  using the natural extension of Gel'fand-Pinsker. The second part $M_{j,2}$ is encoded using a nested QGC as described in the proof of Theorem \ref{thm: QGC MAC with state achievable}. 

\textbf{Codebook Construction:}
\begin{itemize}
\item   For each $j=1,2$ and any $m_{j,1}$  generate $2^{\rho_{j,1}}$ sequences $\mathbf{u}_{j}^n$ randomly and independently according to the distribution $\prod_{i=1}^n p(u_{j,i})$. Such sequences are denoted by $u_j(m_{j,1}, a_j)$, where $a_j\in [1:2^{n\rho_{j1}}]$. The collection of all such codewords is denote by $\mathcal{C}_{j,1}$. 

\item We use a $(n,k_j,l)$-nested QGC as described in the proof of Theorem  \ref{thm: QGC MAC with state achievable}. Denote such nested QGC by $\mathcal{C}_{j,2}$. Let $\mathcal{C}_{I,j}$ be the inner codebook associated to $\mathcal{C}_{j,2}$. Let $2^{n\rho_{j,2}}$ be the size of $\mathcal{C}_{I,j}$. As described in the proof of Theorem \ref{thm: QGC MAC with state achievable}, the codebook $\mathcal{C}_{j,2}$ is divided into $2^{nR_{j,2}}$ bins, where each bin is a shifted version of the inner codebook. Each bin corresponds to a message $m_{j,2}\in [1:2^{nR_{j,2}}]$. Denote such bin by $\mathcal{B}_j(m_{j,2})$.

\item Given the sequences $\mathbf{s}_j \in \mathcal{S}_j^n, \mathbf{u}_j\in \mathcal{U}_j^n$, and $\mathbf{v}_j\in \ZZ_{p^r}^n$ generate a sequence $\mathbf{x}_j$ according to $\prod_{j=1}^n p(x_{j,i}|s_{j,i} u_{j,i}, v_{j,i})$. Denote such sequence by $x_j(\mathbf{s}_j, \mathbf{u}_j, \mathbf{v}_j)$. 

\item For the decoder, we use $\mathcal{C}_{1,1}, \mathcal{C}_{2,1}$ and $\mathcal{D}$ as the codebooks, where  $\mathcal{D}=\mathcal{C}_{1,2}\oplus \mathcal{C}_{2,2}$. Note $\mathcal{D}$ is a $(n, k_1+k_2, l)$ nested QGC. The inner code associated with $\mathcal{D}$ is $\mathcal{C}_{I,1}\oplus \mathcal{C}_{I,2}$. Let $2^{n\rho}$ denote the size of the inner code. There are $2^{n(R_{1,2}+R_{2,2})}$ bins in $\mathcal{D}$. Each bin corresponds to a message pair $(m_{1,2}, m_{2,2})$. 

\end{itemize}
 
\textbf{Encoding:}
The $j$th encoder is given a message  pair $(m_{j,1}, m_{j,2})$ and a state sequence $\mathbf{s}_j$. The $j$th encoder finds  $\mathbf{v}_j\in \mathcal{B}_j(m_{j,2})$ and $a_j\in [1:2^{n\rho_{j1}}]$ such that $( u_j(m_{j,1}, a_j),\mathbf{v}_j, \mathbf{s}_j)\in A_\epsilon^{(n)}(U_j,V_j,S_j) $. If such sequences were found, the $j$th encoder sends $x_j(\mathbf{s}_j, \mathbf{u}_j, \mathbf{v}_j)$, where $\mathbf{u}_j=u_j(m_{j,1}, a_j)$. Otherwise an error is declared.

\textbf{Decoding}:
The decoder receives $\mathbf{Y}^n$ from the channel. The decoding is performed in two stages. In the first stage, the decoder lists all codewords $\mathbf{\tilde{u}}_1\in \mathcal{C}_{1,1}, \mathbf{\tilde{u}}_2\in \mathcal{C}_{2,1}$ such that    $(\mathbf{\tilde{u}}_1,\mathbf{\tilde{u}}_2, Y^n)$ are $\epsilon$- typical with respect to $P_{U_1U_2Y}$. If $\mathbf{\tilde{u}}_1, \mathbf{\tilde{u}}_2$ are unique, the decoder proceeds to the next stage. Otherwise it declares an error. At the next stage, the decoder finds all $\mathbf{\tilde{v}}\in \mathcal{D}$ such that $(\mathbf{\tilde{u}}_1,\mathbf{\tilde{u}}_2, \mathbf{\tilde{v}}, Y^n) \in A_\epsilon^{(n)}( U_1U_2V_1\oplus V_2Y)$. Then the decoder checks if all $\mathbf{\tilde{v}}$ belong to a unique bin associated with $(\tilde{m}_{1,2}, \tilde{m}_{2,2})$. Finally the decoder declares that $(\tilde{m}_{1,1}, \tilde{m}_{1,2}, \tilde{m}_{2,1}, \tilde{m}_{2,2})$ is sent, if it is unique. Otherwise it declares an error.

\textbf{Error Analysis:}
We can show that the probability of error at the encoders is small enough, if the following covering bounds hold
\begin{align*}
\rho_{j,1} &> I(U_j;S_j)\\
\rho_{j,2}& >  \max_{1\leq t \leq r} \frac{H(W_j|\bar{Q})}{H([W_j]_t|\bar{Q})} \big(\log_2 p^t-H([V_j]_t|S_j U_j)\big),
\end{align*}
where $j=1,2$. Also the error at the decoder is small, if the following packing bounds hold
\begin{align*}
R_{1,1}+\rho_{11}&< I(U_1;Y|U_2)\\
R_{2,1}+\rho_{21}&< I(U_2;Y|U_1)\\
R_{1,1}+\rho_{11}+R_{2,1}+\rho_{21}&<I(U_1U_2;Y)+I(U_1;U_2)\\
R_{1,2}+R_{2,2}+\rho &< \log_2p^r-H(V_1\oplus V_2|YU_1U_2),
\end{align*}
where $\rho=\frac{H(V_1\oplus V_2|\bar{Q})}{H(V_j|\bar{Q})}\rho_{j,2}, j=1,2$. Next, we substitute $R_j-R_{j,2}$ for $R_{j,1}, j=1,2$ in the above bounds. Finally, we use the Fourier-Motzkin technique \cite{ElGamal-book} to eliminate $R_{j,2}, \rho_{j,1}, \rho_{j,2}, j=1,2$. This completes the proof. 
\end{proof}

==> proof_of_thm_comp_over_MAC.tex <==
\section{Proof of Theorem \ref{thm: com_over_mac}}\label{sec: proof of achiv_mac}
We need to find conditions for which the probability of the error events $E_1, E_2$ and $E_d$ approach zero. Suppose $\mathbf{G}$ is the generator matrix, and $\mathbf{b}$ is the translation of $\mathcal{C}_{I,1}$ and $\mathcal{C}_{I,2}$.  In addition, suppose $\mathbf{\bar{G}}$ is the generator matrix and $\mathbf{\bar{b}}_i$ is the translation defined for $\bar{\mathcal{C}}_i, i=1,2$. 
 For any $\mathbf{a}\in \ZZ_{p^r}^k$ define the map $\phi(\mathbf{a})=\mathbf{a} \mathbf{G}+\mathbf{b}$. By $\Phi(\cdot)$ denote the map $\phi$ whose matrix and translation are selected randomly and uniformly.   We change the definition of the error event at the decoder. Suppose $\mathbf{x}_i=\phi(\mathbf{w}_i)+b_i$, is the codeword transmitted by encoder $i, i=1,2$. We require the decoder to decode $\mathbf{w}_1+\mathbf{w}_2$. This is a stronger condition, but it is more convenient for error analysis. In what follows, we redefine the decoding operation. Upon receiving $\mathbf{y}$, the decoder finds $\tilde{\mathbf{w}} \in \mathcal{W}_1+\mathcal{W}_2$ such that $\Phi(\tilde{\mathbf{w}})+b_1+b_2$ is jointly typical with $\mathbf{y}$ w.r.t $P_{X_1+X_2,Y}$.  The error event $E$ occurs at the decoder, if  $\tilde{\mathbf{w}}$ is not unique.  Assume $\Phi=\phi, \mathbf{b}_1$ and $\mathbf{b}_2$ are fixed,  the probability of $E$ is  
 \begin{align*}
P(E|  \phi, & \mathbf{b}_1, \mathbf{b}_2)=\sum_{\mathbf{w}_1\in \mathcal{W}_1}\frac{1}{|\mathcal{W}_1|} \sum_{x_1\in \ZZ_{p^r}^n} \mathbbm{1}\{ x_1 = \phi(\mathbf{w}_1)+b_1\} \sum_{\mathbf{w}_2\in \mathcal{W}_2}\frac{1}{|\mathcal{W}_2|} \sum_{x_2\in \ZZ_{p^r}^n} \mathbbm{1}\{ x_2= \phi(\mathbf{w}_2)+b_2\}\\
& \sum_{y\in A_\epsilon^n(Y|x_1,x_2)}  P(y|x_1, x_2) \mathbbm{1}\{ \exists ~ \mathbf{\tilde{\mathbf{w}}} \in  \mathcal{W}  : \mathbf{\tilde{\mathbf{w}}} \neq \mathbf{w}_1+\mathbf{w}_2,   \phi(\mathbf{\tilde{w}})+b_1+b_2 \in A_\epsilon^n(X_1+X_2|y) \}
\end{align*} 
Denote $Z \triangleq X_1+X_2$ with probability one. Also, let  $\mathcal{W} \triangleq \mathcal{W}_1+\mathcal{W}_2$. By upper bounding the last indicator function, we get 

\begin{align*}
P(E | \phi, b_1, b_2) &\leq \sum_{\mathbf{w}_1\in \mathcal{W}_1}\frac{1}{|\mathcal{W}_1|} \sum_{x_1\in\ZZ_{p^r}^n} \mathbbm{1}\{ x_1 = \phi(\mathbf{w}_1)+b_1\} \sum_{\mathbf{w}_2\in \mathcal{W}_2}\frac{1}{|\mathcal{W}_2|} \sum_{x_2\in\ZZ_{p^r}^n} \mathbbm{1}\{ x_2= \phi(\mathbf{w}_2)+b_2\}\\
& \sum_{y\in A_\epsilon^n(Y|x_1,x_2)}  P(y|x_1, x_2) \sum_{\substack{ \mathbf{\tilde{w}}\in \mathcal{W} \\ \mathbf{\tilde{w}} \neq \mathbf{w_1+w_2}}}\sum_{\tilde{z}\in A_\epsilon^n(Z|y)} \mathbbm{1}\{\tilde{z}=\phi(\mathbf{\tilde{w}})+b_1+b_2\}
\end{align*} 

Averaging over $\phi, b_1$ and $b_2$ yields:
\begin{align*}
P_e=\EE\{P(E|\Phi, B_1, B_2)\} \leq &\sum_{w_1\in \mathcal{W}_1}\frac{1}{|\mathcal{W}_1|} \sum_{x_1\in\ZZ_{p^r}^n} \sum_{\mathbf{w}_2\in \mathcal{W}_2}\frac{1}{|\mathcal{W}_2|} \sum_{x_2\in\ZZ_{p^r}^n} \sum_{y\in A_\epsilon^n(Y|x_1,x_2)}  P(y|x_1, x_2) \sum_{\substack{ \mathbf{\tilde{w}}\in \mathcal{W} \\ \mathbf{\tilde{w}} \neq \mathbf{w_1+w_2}}}\sum_{\tilde{z}\in A_\epsilon^n(Z|y)} \\ &P\{\tilde{z}=\Phi(\mathbf{\tilde{w}})+B_1+B_2, x_1 = \Phi(\mathbf{w}_1)+B_1,x_2= \Phi(\mathbf{w}_2)+B_2\}
\end{align*}


Notice that $B_1$ and $B_2$ are uniform over $\ZZ_{p^r}^n$ and independent of other random variables. Hence, the most inner term in the above summations is simplified to
\begin{align}\label{eq: pf comp over MAC - probability}
p^{-2nr} P\{\tilde{z}-x-y=\Phi(\mathbf{\tilde{w}}-(\mathbf{w_1+w_2}))\}
\end{align}
Using  Lemma \ref{lem: P(phi)}, if $\mathbf{\tilde{w}}-(\mathbf{w_1+w_2}) \in H^k_s \backslash H_{s+1}^k$ the expression in \eqref{eq: pf comp over MAC - probability}  equals $p^{-2nr} p^{-n(r-s)}\mathbbm{1}\{\tilde{z}-x-y \in H_s^n\}$, where $ 0\leq s \leq r-1$. Therefore, the probability of error is upper-bounded as 
\begin{align} \label{eq: pe_1}
P_e\leq &\sum_{\mathbf{w_1}\in \mathcal{W}_1}\frac{1}{|\mathcal{W}_1|} \sum_{x_1\in \ZZ_{p^r}^n} \sum_{w_2\in \mathcal{W}_2}\frac{1}{|\mathcal{W}_2|} \sum_{x_2\in \ZZ_{p^r}^n} \sum_{y\in A_\epsilon^n(Y|x_1,x_2)}  P(y|x_1, x_2) \sum_{s=0}^{r-1}\sum_{\substack{ \mathbf{\tilde{w}}\in \mathcal{W} \\ \mathbf{\tilde{w}}-(\mathbf{w_1+w_2}) \in H^{k}_{s}}}\sum_{\substack{\tilde{z}\in A_\epsilon^n(Z|y)\\ \tilde{z}-x-y \in H^n_{s}}} p^{-2nr} p^{-n(r-s)}
\end{align}
Note the most inner term in the above summations does not depend on the value of $\tilde{z}$ and $\mathbf{\tilde{w}}$. Hence, we replace those summations by the size of the corresponding subsets. Using Lemma \ref{lem: typical set intersection subgroup} we can bound the size of these subsets and get the following bound on the probability of error
\begin{align*}
P_e\leq &\sum_{w_1\in \mathcal{W}_1}\frac{1}{|\mathcal{W}_1|} \sum_{x_1\in \ZZ_{p^r}^n} \sum_{w_2\in \mathcal{W}_2}\frac{1}{|\mathcal{W}_2|} \sum_{x_2\in \ZZ_{p^r}^n}  \sum_{y\in A_\epsilon^n(Y|x_1,x_2)}  P(y|x_1, x_2) \sum_{s=0}^{r-1} 2^{kH(W|Q, [W]_s)}~ 2^{n(H(Z|Y[Z]_{s})+c \delta(\epsilon))}p^{-2nr} p^{-n(r-s)},
\end{align*}
where $W=W_1+W_2$, $c$ is a constant, and $\delta(\cdot)$ is the function defined in Lemma \ref{lem: typical set intersection subgroup}. As the terms in the above expression do not depend on the values of $\mathbf{w}_1, \mathbf{w}_2, \mathbf{x}_1, \mathbf{x}_2$ and  $\mathbf{y}$, we can replace the summations over them with the corresponding sets. As a result, we have 
\begin{align*}
P_e\leq &  \sum_{s=0}^{r-1}  p^{-n(r-s)}  2^{kH(W|Q, [W]_s)}~ 2^{n(H(Z|Y[Z]_{s})+c\delta(\epsilon))}
\end{align*}
 Therefore, $P_e$ approaches zero as $n\rightarrow \infty$, if the following bounds hold:
\begin{align}\label{equ: bound simple form}
\frac{k}{n} H(W|Q, [W]_s) \leq   \log_2 p^{r-s}- H(Z|Y[Z]_{s})-c\delta(\epsilon), \quad \mbox{for} ~ 0\leq s\leq r-1.
\end{align}
Since  $X_1+X_2$ is uniform over $\ZZ_{p^r}$, the right-hand side of (\ref{equ: bound simple form}) equals $I(Z;Y|[Z]_s)$. Note by definition $R_1=\frac{1}{n}\log_2 |\mathcal{C}_j|\leq \frac{1}{n}\log_2 |\mathcal{W}_1| \leq \frac{k}{n} H(U|Q)  $. Similarly, $R_2\leq \frac{k}{n} H(V|Q) $. Therefore, these inequalities along with (\ref{equ: bound simple form}) give,
\begin{align*}
R_i \leq \frac{H(W_i|Q)}{H(W_1+W_2|Q, [W_1+W_2]_s) } (I(X_1+X_2;Y|[X_1+X_2]_s)-c\delta(\epsilon), ~ i=1,2.
%R_2 \leq \frac{H(V|Q)}{H(W|Q, [W]_s) } I(X_1+X_2;Y|[X_1+X_2]_s).
\end{align*}
We take the union of the above region over all possible PMFs $p(w_1,w_2,q)=p(q)p(w_1|q)p(w_2|q)$, where $p(q)$ is a rational number. Since rational numbers are dense, we can let the PMF of $Q$ be an arbitrary PMF on $\mathcal{Q}$. Using the same argument as in Lemma \ref{lem: cardinality of Q}, we can bound the cardinality of $Q$ by  $|\mathcal{Q}| \leq r$. 

